Recursive Augmented Fernet (RAF) Token: Alleviating the Pain of Stolen Tokens

A robust authentication and authorization mechanism is imperative in modular system development, where modularity and modular thinking are pivotal. Traditional systems often employ identity modules responsible for authentication and token issuance. Tokens, representing user credentials, offer advantages such as reduced reliance on passwords, limited lifespan, and scoped access. Despite these benefits, the "bearer token" problem persists, leaving systems vulnerable to abuse if tokens are compromised. We propose a token-based authentication mechanism addressing modular systems' critical bearer token problem. The proposed mechanism includes a novel RAF (Recursive Augmented Fernet) token, a blacklist component, and a policy enforcer component. RAF tokens are one-time-use tokens, like tickets. They carry commands, and the receiver of an RAF token can issue new tokens using the received RAF token. The blacklist component guarantees an RAF token can not be approved more than once, and the policy enforcer checks the compatibility of commands carried by an RAF token. We introduce two variations of RAF tokens: User-tied RAF, offering simplicity and compatibility, and Fully-tied RAF, providing enhanced security through service-specific secret keys. We thoroughly discuss the security guarantees, technical definitions, and construction of RAF tokens backed by game-based proofs. We demonstrate a proof of concept in the context of OpenStack, involving modifications to Keystone and creating an RAFT library. The experimental results reveal minimal overhead in typical scenarios, establishing the practicality and effectiveness of RAF. Our experiments show that the RAF mechanism beats the idea of using short-life Fernet tokens while providing much better security.

==> code.tex <==
\section{Code}
Code on Github:
\href{https://github.com/rahaeimehr/RAFT}{RAFT} 

==> codes/IssueRaft.tex <==
\begin{code}
\caption{The source code for Issuing a RAFT.}
\label{code:issueRAFT}
\scriptsize
\begin{minted}[breakanywhere]{python}

import os
import time
from cryptography.hazmat.backends import default_backend
import base64
from cryptography import fernet
from cryptography.hazmat.primitives.hmac import HMAC
from cryptography.hazmat.primitives import hashes
from cryptography import utils
from struct import pack,unpack, unpack_from

class RAFT(object):
    _lifeTime = 10
    def __init__(self, parent_token=None, backend=None):
        if backend is None:
            backend = default_backend()
        self._backend = backend

        if parent_token is not None:
            self.SetParentToken(parent_token)

    def SetParentToken(self,parent_token):
        self._parentToken = base64.urlsafe_b64decode(parent_token)
        self._signKey = self._parentToken[-32:-16]
        self._encryptionKey = self._parentToken[-16:]
        self._id = self._parentToken[:-32]

    def SetCommand(self, command):
        self._command = command

    def Finalize(self, life_time = None):
        if life_time is not None:
            self._lifeTime = life_time

        self._NewToken = pack(">BH" + 
                              str(len(self._id))+"s",
                              0x91,
                              len(self._id),
                              self._id)
        self._command=pack(">Q8s"+str(len(self._command))+"s", int(time.time())+self._lifeTime,os.urandom(8),self._command) #bytearray(self._command,"utf8")
        self._NewToken+=self._command
        self.h = HMAC(self._signKey, hashes.SHA256(), self._backend)
        self.h.update(self._NewToken)
        self._NewToken += self.h.finalize()
        return base64.urlsafe_b64encode(self._NewToken)
\end{minted}
\end{code}        

==> codes/JWSToken.tex <==
\begin{code}
\caption{An example of a JWS token, its header and payload.}
\label{code:jwsToken}
\scriptsize
\begin{minted}[breakanywhere]{bash}
Token=eyJhbGciOiJIUzI1NiIsInR5cCI6IkpXVCJ9.eyJvcGVuc3RhY2tfcHJvamVjdF9pZCI6Ijg3NjMwZGZhNzgwMWEwOTExMTEwOTgzNDcyM2JjYTk1Iiwic3ViIjoiM2ZlMTUxMTNjZjc5NGU4ZjljNWRhZDlmMTA3M2IwODkiLCJleHAiOjE1NzEyMzU0NDEsIm9wZW5zdGFja19hdWRpdF9pZHMiOlsibXpRUTkyQ2JBNzg5YWE3ODkyODgyOCJdLCJpYXQiOjE1NzEyMzMzNTEsIm9wZW5zdGFja19tZXRob2RzIjpbInBhc3N3b3JkIl19.kIjoiODc2MzBkZmE3OGFzZHF3MDFhMDkxMTExMDk4MzQ3MjNiY2E5NSIsInN1YiI6IjNmZTE1MTEzc2RzZH_fw=
header={
  "alg": "HS256",
  "typ": "JWT"
}
payload={
    "openstack_project_id":"87630dfa7801a09111109834723bca95",
    "sub":"3fe15113cf794e8f9c5dad9f1073b089",
    "exp": 1571235441,
    "openstack_audit_ids":["mzQQ92CbA789aa78928828"],
    "iat": 1571233351,
    "openstack_methods": ["password"]
}
\end{minted}
\end{code}

==> codes/fernet.tex <==
\begin{code}
\caption{An example of a Fernet Key, a Fernet token, and the payload of the token.}
\label{code:projectScopedToken}
\scriptsize
\begin{minted}{bash}
token="gAAAAABdpxhmvMe_byl3qKlJ0KVXizdSyL_38Idxam2ap7O1T9_xzX9eVJ6WCozRKlXjH6oZlDuOyS0nI_57u0G0ceOt7coUtDPPI1TipydgxMekVNtbhdHuR8A9BMvY1pPAVkGV_23Hd_Ste0eiTXP7m_7W77Vj3X2qGkjkeuinyGZsTclYZOc"

key="Qh4ZzunoX36Ri0TKVa3bXqzTQKzwqT3G4JfmGw1ZNtU="

payload={
    "audit_ids": ["JGyyhGnrSfGaGCaY4VV30w"],
    "expires_at": "2019-10-16T14:17:26.000000Z",
    "project id": "08b72d6e4f2b465d96e9e0db2f10d232",
    "user id": "4df1c1afd84544d0af9094e023811529"
}
\end{minted}
\end{code}

==> codes/fernetToken.tex <==
\begin{code}
\caption{An example of a Fernet Key, a Fernet token, and the payload of the token.}
\label{code:projectScopedToken}
\scriptsize
\begin{minted}{bash}
token="gAAAAABdpxhmvMe_byl3qKlJ0KVXizdSyL_38Idxam2ap7O1T9_xzX9eVJ6WCozRKlXjH6oZlDuOyS0nI_57u0G0ceOt7coUtDPPI1TipydgxMekVNtbhdHuR8A9BMvY1pPAVkGV_23Hd_Ste0eiTXP7m_7W77Vj3X2qGkjkeuinyGZsTclYZOc"

key="Qh4ZzunoX36Ri0TKVa3bXqzTQKzwqT3G4JfmGw1ZNtU="

payload={
    "audit_ids": ["JGyyhGnrSfGaGCaY4VV30w"],
    "expires_at": "2019-10-16T14:17:26.000000Z",
    "project id": "08b72d6e4f2b465d96e9e0db2f10d232",
    "user id": "4df1c1afd84544d0af9094e023811529"
}
\end{minted}
\end{code}

==> codes/payloadForScopedToken.tex <==
\begin{code}
\caption{The required payload for getting a scoped token}
\label{code:payloadForScopedToken}
\scriptsize
\begin{minted}[breakanywhere]{bash}
{ 
 "auth": {
   "identity": { 
     "methods": ["password"],"password": {
       "user": {
         "domain": {
           "name": "$OS_USER_DOMAIN_NAME"
           }, "name": "$OS_USERNAME",
           "password": "$OS_PASSWORD"
         } 
       } 
     },"scope":{
       "project": {
         "domain": { 
           "name": "$OS_DOMAIN_NAME" 
         },"name":  "$OS_PROJECT_NAME" 
       } 
     }
}
\end{minted}
\end{code}

==> codes/uuid.tex <==
\begin{code}
\caption{A sample UUID token.}
\label{code:UUIDToken}
\scriptsize
\begin{minted}{bash}
598aed93fefa7bd1c4821fbc53a8b32f
\end{minted}
\end{code}

==> codes/uuidToken.tex <==
\begin{code}
\caption{A sample UUID token.}
\label{code:UUIDToken}
\scriptsize
\begin{minted}{bash}
598aed93fefa7bd1c4821fbc53a8b32f
\end{minted}
\end{code}

==> codes/validateRAFT.tex <==
\begin{code}
\caption{The source code for Validating a RAFT.}
\label{code:validateRAFT}
\scriptsize
\begin{minted}[breakanywhere]{python}

import os
import time
from cryptography.hazmat.backends import default_backend
import base64
from cryptography import fernet
from cryptography.hazmat.primitives.hmac import HMAC
from cryptography.hazmat.primitives import hashes
from cryptography import utils
from struct import pack,unpack, unpack_from

class RAFT(object):
    _lifeTime = 10
    def __init__(self, backend=None):
        if backend is None:
            backend = default_backend()
        self._backend = backend

    def GetKey(self, token):
        v, = unpack_from(">B",token,0)
        if v==0x91 :
            lenId, = unpack_from(">H",token,1)
            OriginalId, = unpack_from(">" + str(lenId)+"s", token,3)
            cmd = token[19+lenId:]
            print(cmd)
            keys, cmds = self.GetKey(OriginalId)
            cmds.append(cmd)
            sign_key = keys[:16]
            h = HMAC(sign_key, hashes.SHA256(), self._backend)
            h.update(token)  
            hmac=h.finalize()
            return hmac, cmds
        else:
            sign_key = base64.urlsafe_b64decode(FernetKey)[:-16]
            h = HMAC(sign_key, hashes.SHA256(), self._backend)
            h.update(token)            
            return h.finalize(),[]
        return ""
        
    def ValidateRAFT(self, token):
        token = base64.urlsafe_b64decode(token)
        v, = unpack_from(">B",token,0)
        if v==0x91 :
            lenId, = unpack_from(">H",token,1)
            OriginalId, =  unpack_from(">"+str(lenId)+"s",token,3)
            cmd = token[19+lenId:-32] 
            keys,cmds = self.GetKey(OriginalId)
            cmds.append(cmd)
            sign_key = keys[:16]
            h = HMAC(sign_key, hashes.SHA256(), self._backend)
            h.update(token[:-32])  
            hmac=h.finalize()
            if hmac== token[-32:]:
                return True,cmds
            else:
                raise Exception("Error: Not a RAFT token (MAC)")
        else:
            raise Exception("Error: Not a RAFT token (Format)")
        return ""
\end{minted}
\end{code}                

==> sections/FromCCS.tex <==
\section{Improved Tokening Mechanism}
\label{sec:improvement}

Our analysis has shown that the simulator of the ideal cloud cannot emulate the corrupted services unless we relax the security promises of the ideal cloud.
To a large extent, these concerns arise due to the use of bearer tokens, which enable anyone who can see a token to masquerade as corresponding user and perform any action allowed to the owner of the token on behalf of him.
Bearer-tokens are leaked to the adversary in both partially and fully corrupted services which could happen through a vulnerability.
Once a service corrupted, it could be malicious in at least two important ways:
\begin{itemize}
\item A service can use a token to obtain unrequested services charged to the user.
\item A service can use a token to access other resources at another service (like exporting a disk with sensitive information).
\end{itemize}

The above problems are not tolerated by the cloud users. Having a bug free cloud is not realistic, but reducing effects of buggy code is possible. Therefore, it is desired to have OpenStack guarantee the modularity security requirement defined as follows:

%\rc{2118 why "minimum"?   this is the new requirement on top of the legacy system, right? so maybe "new security guarantee"?   also maybe cans strengthen the guarantee, to cover other operations as well?}
%\rr{I changed the term to ``Modularity Security Requirement''. Is that good? }
%\mv{I might have used the word ``isolation'' but I defer to the will of the crowd.}

\theoremstyle{definition}
\newtheorem{minsec}{Definition} 
\begin{minsec}
\textit{Modularity Security Requirement}: If an adversary corrupts a service, other services just do whatever requested to do by the users, nothing more. For example, if an adversary corrupts the Image service, he cannot create or delete a node, but if a user issues a ``create node'' command, it is possible to create a node with a corrupted image because of the image service corruption.
\end{minsec}


%\mv{Another advantage of one time tokens that we should highlight: all non-Keystone services don't need to have a ``secure token deletion'' mechanism,  good because they are admittedly tough to build properly!}

We propose to limit the impact of service corruption by preventing replay attacks and scoping tokens only to handle the request desired by the user (following an idea laid out in \cite{sze2016hardening,desnoyers_using_2015}).
As a result, even if an attacker captures a credential submitted to a non-Keystone service by an honest user, he cannot do anything more on behalf of the user. In the following, we explain our two proposals for the OpenStack token issue which improve current security guarantees: 1) Ticketing System, and 2) Recursive Augmented Fernet Tokens.

A one-time use token scoped to a specific job resembles a ``ticket'' as used in Kerberos \cite{SteinerNS88} or in TLS 1.3's zero round trip time mechanism \cite{KrawczykW16}.

\subsection{RAFTs}
\label{sub:raft}

The main drawback of the ticketing system is that a major change must be made to OpenStack to implement it.  Here, we propose a new, backwards-compatible Fernet extension that we call Recursive Augmented Fernet Tokens (RAFTs), on top of which user-specified restrictions can float independently without requiring additional Keystone interaction. The RAFT token mechanism provides the modularity security requirement in the presence of one or more corrupted services just as ticketing accomplished. Fundamentally, RAFTs use the Fernet HMAC as a shared secret between the user and Keystone that can be used to authenticate arbitrary user-supplied restrictions.    

The Fernet token is a recent innovation that uses cryptography to provide authenticity without accessing a central DB. It is a mechanism by which Keystone creates a private, authenticated channel to itself. It has quickly become the preferred token format for OpenStack as it does not require maintaining a central database of valid tokens, which would add network load and complexity when running a distributed Keystone service (cf.~\S \ref{sec:multi}). The current Fernet token mechanism is \cite{fernet}. The Fernet token is represented as follows:
%
\newcommand{\HMAC}{\textit{HMAC}}
\newcommand{\spec}{\textit{Specification}}
\newcommand{\rest}{\textit{Restrictions}}
\newcommand{\req}{\textit{Request}}
\newcommand{\token}{\textit{Token}}
\newcommand{\fernetToken}{\token_{\textit{Fernet}}}
\newcommand{\otoken}{\textit{OldToken}}
\begin{align*}
Sk &= \text{Keystone signing key} \\
\fernetToken &= \spec \parallel \HMAC_{Sk}(\spec) \\
\end{align*}
%
Because the original Fernet token is a bearer one, the link between the user and Keystone must be authenticated and encrypted to ensure that only the user receives $\fernetToken$ from Keystone.

In RAFT, a user first obtains a Fernet token from Keystone. The user takes the $\HMAC_{Sk}(\spec)$ as a shared secret key $Uk$ between Keystone and himself. Then, for each of his subsequent requests, the user calculates:
%
\newcommand{\raftToken}{\token_{\textit{RAFT}}}
\begin{align*}
\raftToken   =&\req	 \parallel \\
			  &\spec \parallel  \\
              &\rest \parallel \\
              &\HMAC_{Uk}(\req \parallel \spec \parallel \rest)
\end{align*}
The \rest{} could be a composition of anything like a shortened expiration time (``expiration-time $ = 5$ secs'') or endpoint restrictions (``service=cinder'').
The RAFT token is a self-explained token and the user request is part of the token and there is no need to accompany the request with the token. Hence, the user just sends the RAFT token to the desired service. For the sake of backward compatibility, which we will talk about later, all the services also continue to accept job requests in the format of $(\req,Token)$. 

\newcommand{\srvid}{\textit{ServiceId}}
When a service receives $\raftToken$, the service forwards it to Keystone asking for validation. If the answer of Keystone was ``valid'', the service extracts the \req{} and \rest{} from the token and gets the work done accordingly.

In the current OpenStack architecture, each service gets a service token from Keystone. The service token is used to authenticate the service to other services \cite{service-token}. RAFT replaces this bearer token as well: the token of a service is never sent to other services, but is instead used as a signing key $Svk$ in the RAFT framework.
Concretely, if a service needs to involve other services, then it calculates:
\newcommand{\newRaftToken}{New\_\raftToken}
\begin{align*}
Svk =& \text{Service signing key, from Keystone} \\
\newRaftToken =&\raftToken \parallel \\
		             &\rest \parallel \\
		             &\srvid \parallel \\                     
              		 &\HMAC_{Svk}(\raftToken \parallel \rest),
\end{align*}
and sends the result to the required services. We highlight three tangible benefits of this method:
each service is able to add (but not remove!) \rest{} to the user's token,
the MAC
%provides end-to-end verifiability from its creation at the original service until its verification at Keystone; as a consequence, it
authenticates the channel used to make a service-to-service request,
and
the token provides the recipient service with the provenance of the request \cite{service-token}.

% \kh{I have been assuming authentication for services. e.g. if storage receives and attach/detach request from anyone other than compute it will drop it (b/c we want them to agree on state - I don't think the tokening totally solves this because then a corrupted user could initiate a request with storage instead of compute and could get a weird system state from it (volume thinks it's attached, but node doesn't)}

% \mv{Kyle, I think we actually agree here. There is a need for service-to-service authentication. My point is that the tokens allow us to bootstrap this. It's not just the user token; it is also the service tokens that help here.}

% When a service receives $\svtoken_{RAFT}$, it follows the same steps as above, except when it needs to involve other services, the service must replace its own id and signature with the previous one in the token. 

When Keystone receives a token validation request from a service $S$ for token $T$, it follows the Fernet protocol as if $T$ is a Fernet token. Keystone looks into its blacklist to see whether $T$ was used by $S$ or not. If yes, Keystone returns fail. Otherwise, Keystone validates all the service signatures. Then, it takes out \spec{} from $T$ and calculates $HMAC_{Sk}(\spec)$ as its signing key. Using the result, Keystone is able to verify the user's signature embedded into $T$, too. If the token is valid, Keystone adds $(T,S)$ to its blacklist and returns ``valid''. Just as in the ticketing system, the expiration time of RAFT tokens are very short. Therefore, the blacklist can be implemented in a lightweight memcached structure.

The RAFT is specified fully in Algorithm \ref{alg:RAFT}.

% \input{algorithm-raft}


\paragraph{Pros and cons.}
RAFT uses the Fernet token to create a user to keystone private/authenticated channel, while not jeopardizing keystone's existing channel to itself. It can be implemented in a backward compatible way. RAFT tokens are larger than Fernet tokens and the size of buffers used for storing tokens in different OpenStack modules must be carefully inspected.


\subsection{Effect of One-Time Tokens on Corruption} 


Restricting tokens to be single use with specific parameters limits the scope of adversarial corruptions. Previously a corrupted service could store all tokens it sees and use them at will. This modification ensures that once a token has been used it will not be accepted again in the future. Additionally, since tokens are scoped, it is not possible for a corrupted service to lie to uncorrupted services about the content of a user's request. Specifically, users will indicate when requesting a token exactly which of their resources it grants access to. This would not prevent a corrupted Compute from deleting a node when a user had asked to create one or creating a node with a completely different specification since Compute could simply do these things without bothering to verify the token, but it \textit{would} prevent Compute from requesting a different image from the Image service than the one the user had intended. This helps in the case where the adversary has not already seen, via a request by a different user, the image it would like to have Compute use. 
Scoped, single use tokens even benefit functionalities that go beyond those captured in our model; for example, an adversary who corrupted the Compute service would be unable to upload arbitrary images.

We also remark that there is another notion of limited-use tokens with a security-performance tradeoff.
Many OpenStack engineers desire a stateless Keystone architecture in order to distribute the authentication process over several servers and improve scalability and performance.
If it is desirable to keep Keystone stateless, then one could instead design ``limited-reuse'' tokens with a short lifetime. While one could model the impacts of limited reuse by combining rate limiting with a UC model of network time \cite{CanettiHMV17}, in this paper we focus on the One-Time token presented above with an explicit blacklist to prevent reuse. In this setting, we can prove the following theorem.
%The ticketing system keeps a whitelist of services that are allowed to use each token. Conversely, RAFT stores a blacklist of services which have used a token. 

\begin{theorem}\label{lessleaky}
The strengthened version of OpenStack Services using RAFT
securely realizes the less-leaky version of \ic in Algorithm \ref{alg:IdealCloudCorruptonetime} (in Appendix \ref{sec:appendix-onetime-token}) in the (\sexternalnet, \ssmt)-hybrid model. 
\end{theorem}

Appendix \ref{sec:appendix-sim-onetime} formally encodes the simulator demonstrating that the services UC-realize this new ideal cloud. Appendix \ref{sec:proof} provides the proof of UC emulation.

%\rc{how did our analysis show this? ie, say which properties of the ideal cloud enable the analysis - and explain the implications re the security.}
%\mv{I agree. We need to be specific about \emph{what} improves from one ideal cloud model to the other. I wrote some flowery text below but there is no substance here yet. (Maybe also put some of the high-level takeaways at the beginning of this section as well.}

Juxtaposing the ideal clouds in the bearer token (Algorithm \ref{alg:IdealCloudCorrupt}) and One-Time token (Algorithm \ref{alg:IdealCloudCorruptonetime}) scenarios is quite illustrative. An OpenStack developer who might not understand the full complexity of UC (and thus who might ignore our simulators and proofs) can still compare those two algorithms to understand the harms of partial compromise in the two settings. For example, Algorithm \ref{alg:IdealCloudCorrupt} shows that a corrupted \sblock can tamper with the delivery of an image from \simage to \scompute during a Create Node operation in the bearer token model, whereas Algorithm \ref{alg:IdealCloudCorruptonetime} shows that the same attack is not possible in the ideal cloud for the One-Time token model.

Furthermore, the simulator in the scoped one-time token model is more stringent than the simulator in the unscoped bearer token model. To enforce the single-use constraint, \s creates a black list to store the services that have already checked the validity of a credential using \ssid; the simulator then rejects all future attempts to validate the same credential. To enforce the scoping constraint, \s only issues credentials when given both an \ssid \emph{and} a request scope; the simulator records this intended scope and subsequently rejects all attempts to validate the credential in pursuit of a request outside of this scope.
% MV: Old version of the 2nd half of this paragraph below.
%In the single-use setting, \s creates and stores one credential per \ssid and request scope; \s also stores a black list for each \ssid to store the services that have already made a valid validation request using \ssid. The simulator adds the services that have made valid validation request to the $BlackList_{\ssid}$ and therefore does not allow any further request with the same \ssid for that service. In addition, the simulator stores the scope of the request and whenever a request is made with the same \ssid, the simulator makes sure that the request falls into the scope of the token otherwise rejects it.


%Differences between bearer token and one time token from simulator's perspective:
%Bearer token is an unscoped and multi used token, therefore, if the credential of a user is compromised, the adversary is able to get access to any project that the user is able to access. To model this, the simulator creates and stores credential per each compromised \uid. However, in the one time token, because of its scope and one time usage property, if a token is compromised, the adversary may only used it to get access to stuffs that are defined in the token. In addition, the adversary is not able to use the same token to make more that one request to a service. To realize these properties, the simulator is not storing credential per user any more; instead it creates and stores credential per\ssid, stores request's scope, and creates a black list per each \ssid to store the services which made a valid validation request using \ssid.
%With these changes, the simulator is able to act differently for these two different mechanism. That is, for bearer token, the simulator does not check or store information related the number of time a service makes valid validation request for the same \uid and since the token does not have scope, the simulator response to any request which diverges from the original request but has valid validation.
%On the other hand, in the one-time token, the simulator stores the services that have made valid validation request and does not allow any further request with the same \ssid for that service. In addition, the simulator stores the scope of the request and whenever an request is made with the same \ssid, the simulator makes sure that the request falls into the scope of the token otherwise rejects it.



%Another advantage of one time tokens that we should highlight: all non-Keystone services don't need to have a ``secure token deletion'' mechanism,  good because they are admittedly tough to build properly

More generally, the UC ideal cloud that models any suggested security improvement permits OpenStack developers to understand concretely the value added by this improvement.
This is an example for how UC modeling can provide developers with a valuable new tool that they can use to balance the relative importance of addressing any of the numerous bug reports on their plate at any given time.



%below are random notes
\iffalse
https://www.lbragstad.com/blog/fernet-tokens-and-key-distribution
https://www.lbragstad.com/fernet-tokens-and-key-rotation/
https://platform9.com/blog/platform9-distributed-keystone-architecture/
\fi




==> sections/background.tex <==
\section{Background}
\begin{Verbatim}[breaklines]
Fernet tokens
The fernet token format was introduced in the OpenStack Kilo release and now is the default token provider in Keystone. Unlike the other token types mentioned in this document, fernet tokens do not need to be persisted in a back end. AES256 encryption is used to protect the information stored in the token and integrity is verified with a SHA256 HMAC signature. Only the Identity service should have access to the keys used to encrypt and decrypt fernet tokens. Like UUID tokens, fernet tokens must be passed back to the Identity service in order to validate them. For more information on the fernet token type, see the Fernet - Frequently Asked Questions.

A deployment might consider using the fernet provider as opposed to JWS tokens if they are concerned about public expose of the payload used to build tokens.

JWS tokens
The JSON Web Signature (JWS) token format is a type of JSON Web Token (JWT) and it was implemented in the Stein release. JWS tokens are signed, meaning the information used to build the token ID is not opaque to users and can it can be decoded by anyone. JWS tokens are ephemeral, or non-persistent, which means they won’t bloat the database or require replication across nodes. Since the JWS token provider uses asymmetric keys, the tokens are signed with private keys and validated with public keys. The JWS token provider implementation only supports the ES256 JSON Web Algorithm (JWA), which is an Elliptic Curve Digital Signature Algorithm (ECDSA) using the P-256 curve and a SHA-256 hash algorithm.

A deployment might consider using JWS tokens as opposed to fernet tokens if there are security concerns about sharing symmetric encryption keys across hosts. Note that a major difference between the two providers is that JWS tokens are not opaque and can be decoded by anyone with the token ID. Fernet tokens are opaque in that the token ID is ciphertext. Despite the JWS token payload being readable by anyone, keystone reserves the right to make backwards incompatible changes to the token payload itself, which is not an API contract. We only recommend validating the token against keystone’s authentication API to inspect its associated metadata. We strongly discourage relying on decoded payloads for information about tokens.    
\end{Verbatim}

\subsection{Fernet Token}
Useful link(s):
\begin{description}

%\item \href{https://blog.dolphm.com/openstack-keystone-fernet-tokens/}{OpenStack Keystone Fernet tokens}
%\rr{It is not available now.}

\item \href{https://blog.dolphm.com/inside-openstack-keystone-fernet-token-payloads/}{Fernet token payloads}
\item \href{https://specs.openstack.org/openstack/keystone-specs/specs/keystone/stein/json-web-tokens.html}{jws token}
\end{description}
In April 2015, the OpenStack community introduced Kilo, which one of its main advantages was supporting Fernet token. 
Fernet was originally a secure messaging format created by Heroku in 2013. The OpenStack implementation of this lightweight and more API-friendly format was developed by the OpenStack Keystone core team.
%In 2013, a cloud provider company Heroku introduced Fernet tokens for issuing API requests between remote servers. 
Fernet tokens are message packed tokens that contain authentication and authorization data. Fernet tokens are signed and encrypted before being handed out to users. Most importantly, however, Fernet tokens are ephemeral. This means they do not need to be persisted across clustered systems in order to successfully be validated.




